ABEONA: an Architecture for Energy-Aware Task Migrations from the Edge to the Cloud

This paper presents our preliminary results with ABEONA, an edge-to-cloud architecture that allows migrating tasks from low-energy, resource-constrained devices on the edge up to the cloud. Our preliminary results on artificial and real world datasets show that it is possible to execute workloads in a more efficient manner energy-wise by scaling horizontally at the edge, without negatively affecting the execution runtime.

==> futurework.tex <==
\vspace{-5pt}
\section{Future Work}
\vspace{-5pt}
\label{sec:futurework}

We intend to further investigate the effects observed in our evaluation including a more diverse set of nodes and workloads.
We will investigate the impacts of {CPU} frequency scaling in our results, and how to exploit that in \sys.

%Additionally, whenever a better suited deployment setting is detected or predicted, tasks (including their potential current state) should be migrated to their appropriated location.
We plan to support task migration across heterogeneous nodes within and across layers whenever a better suited deployment setting is detected or predicted.

Finally, we will investigate security aspects within \sys, for applications operating on private data, by leveraging a mix of Intel SGX and ARM~TrustZone nodes.
%\vs{In this case, the control may make the nodes in the edge/fog/cloud unsuitable for execution, effectively migrating the task}
